Bolt-on Differential Privacy for Scalable Stochastic Gradient Descent-based Analytics

While significant progress has been made separately on analytics systems for scalable stochastic gradient descent (SGD) and private SGD, none of the major scalable analytics frameworks have incorporated differentially private SGD. There are two inter-related issues for this disconnect between research and practice: (1) low model accuracy due to added noise to guarantee privacy, and (2) high development and runtime overhead of the private algorithms. This paper takes a first step to remedy this disconnect and proposes a private SGD algorithm to address \emph{both} issues in an integrated manner. In contrast to the white-box approach adopted by previous work, we revisit and use the classical technique of {\em output perturbation} to devise a novel "bolt-on" approach to private SGD. While our approach trivially addresses (2), it makes (1) even more challenging. We address this challenge by providing a novel analysis of the $L_2$-sensitivity of SGD, which allows, under the same privacy guarantees, better convergence of SGD when only a constant number of passes can be made over the data. We integrate our algorithm, as well as other state-of-the-art differentially private SGD, into Bismarck, a popular scalable SGD-based analytics system on top of an RDBMS. Extensive experiments show that our algorithm can be easily integrated, incurs virtually no overhead, scales well, and most importantly, yields substantially better (up to 4X) test accuracy than the state-of-the-art algorithms on many real datasets.

==> Makefile <==
### Makefile --- 

TARGETS = paper

%: %.tex
	latexmk -g -pdf -silent $@ # generate pdf
	latexmk -c $@ # clean up regeneratable files

all: pdf

pdf: ${TARGETS}

clean:
	@echo cleaning up...
	rm -f *.fdb_latexmk *.ps *.dvi *.aux *.bbl *.blg *.brf *.cb *.cb2 \
		 *.idx *.ilg *.ind *.inx *.log *.mpx *.toc *.out *.pstex_t \
		 *.fig.bak  *.ps_e *~ *.tex.* *.thm *.fls



==> figs/Makefile <==
### Makefile --- 

TARGETS = bismarckprivatesgd_tikz

%: %.tex
	pdflatex --jobname=$@_f1 $@.tex
	make -C ../

all: pdf

pdf: ${TARGETS}

clean:
	@echo cleaning up...
	rm -f *.fdb_latexmk *.ps *.dvi *.aux *.bbl *.blg *.brf *.cb *.cb2 \
		 *.idx *.ilg *.ind *.inx *.log *.mpx *.toc *.out *.pstex_t \
		 *.fig.bak  *.ps_e *~ *.tex.* *.thm *.fls


==> plots/covertype/Makefile <==
### Makefile --- 

TARGETS = test1_1_pass test1_10_pass test1_20_pass \
	  test2_1_pass test2_10_pass test2_20_pass \
	  test3_1_pass test3_10_pass test3_20_pass \
	  test4_1_pass test4_10_pass test4_20_pass

%: %.tex
	latexmk -g -pdf -silent $@ # generate pdf
	latexmk -c $@ # clean up regeneratable files

all: pdf

pdf: ${TARGETS}

clean:
	@echo cleaning up...
	rm -f *.fdb_latexmk *.ps *.dvi *.aux *.bbl *.blg *.brf *.cb *.cb2 \
		 *.idx *.ilg *.ind *.inx *.log *.mpx *.toc *.out *.pstex_t \
		 *.fig.bak  *.ps_e *~ *.tex.* *.thm *.fls



==> plots/mnist/Makefile <==
### Makefile --- 

TARGETS = convex_num_passes strongly_convex_num_passes convex_mb \
	test1_1_pass_1_mb  test1_10_pass_1_mb  test1_20_pass_1_mb \
	test1_1_pass_10_mb test1_10_pass_10_mb test1_20_pass_10_mb \
	test1_1_pass_50_mb test1_10_pass_50_mb test1_20_pass_50_mb \
	test2_1_pass_1_mb  test2_10_pass_1_mb  test2_20_pass_1_mb \
	test2_1_pass_10_mb test2_10_pass_10_mb test2_20_pass_10_mb \
	test2_1_pass_50_mb test2_10_pass_50_mb test2_20_pass_50_mb \
	test3_1_pass_1_mb  test3_10_pass_1_mb  test3_20_pass_1_mb \
	test3_1_pass_10_mb test3_10_pass_10_mb test3_20_pass_10_mb \
	test3_1_pass_50_mb test3_10_pass_50_mb test3_20_pass_50_mb \
	test4_1_pass_1_mb  test4_10_pass_1_mb  test4_20_pass_1_mb \
	test4_1_pass_10_mb test4_10_pass_10_mb test4_20_pass_10_mb \
	test4_1_pass_50_mb test4_10_pass_50_mb test4_20_pass_50_mb \

%: %.tex
	latexmk -g -pdf -silent $@ # generate pdf
	latexmk -c $@ # clean up regeneratable files

all: pdf

pdf: ${TARGETS}

clean:
	@echo cleaning up...
	rm -f *.fdb_latexmk *.ps *.dvi *.aux *.bbl *.blg *.brf *.cb *.cb2 \
		 *.idx *.ilg *.ind *.inx *.log *.mpx *.toc *.out *.pstex_t \
		 *.fig.bak  *.ps_e *~ *.tex.* *.thm *.fls



==> plots/old/Makefile <==
### Makefile --- 

TARGETS = accuracy-1 accuracy-10 accuracy-50 \
	accuracy-bst14-1 accuracy-bst14-2 accuracy-bst14-4

%: %.tex
	latexmk -g -pdf -silent $@ # generate pdf
	latexmk -c $@ # clean up regeneratable files

all: pdf

pdf: ${TARGETS}

clean:
	@echo cleaning up...
	rm -f *.fdb_latexmk *.ps *.dvi *.aux *.bbl *.blg *.brf *.cb *.cb2 \
		 *.idx *.ilg *.ind *.inx *.log *.mpx *.toc *.out *.pstex_t \
		 *.fig.bak  *.ps_e *~ *.tex.* *.thm *.fls



==> plots/protein/Makefile <==
### Makefile --- 

TARGETS = test1_1_pass test1_10_pass test1_20_pass \
	  test2_1_pass test2_10_pass test2_20_pass \
	  test3_1_pass test3_10_pass test3_20_pass \
	  test4_1_pass test4_10_pass test4_20_pass

%: %.tex
	latexmk -g -pdf -silent $@ # generate pdf
	latexmk -c $@ # clean up regeneratable files

all: pdf

pdf: ${TARGETS}

clean:
	@echo cleaning up...
	rm -f *.fdb_latexmk *.ps *.dvi *.aux *.bbl *.blg *.brf *.cb *.cb2 \
		 *.idx *.ilg *.ind *.inx *.log *.mpx *.toc *.out *.pstex_t \
		 *.fig.bak  *.ps_e *~ *.tex.* *.thm *.fls


